xCodeEval: A Large Scale Multilingual Multitask Benchmark for Code Understanding, Generation, Translation and Retrieval

Recently, pre-trained large language models (LLMs) have shown impressive abilities in generating codes from natural language descriptions, repairing buggy codes, translating codes between languages, and retrieving relevant code segments. However, the evaluation of these models has often been performed in a scattered way on only one or two specific tasks, in a few languages, at a partial granularity (e.g., function) level, and in many cases without proper training data. Even more concerning is that in most cases the evaluation of generated codes has been done in terms of mere lexical overlap with a reference code rather than actual execution. We introduce xCodeEval, the largest executable multilingual multitask benchmark to date consisting of $25$M document-level coding examples ($16.5$B tokens) from about $7.5$K unique problems covering up to $11$ programming languages with execution-level parallelism. It features a total of $7$ tasks involving code understanding, generation, translation and retrieval. xCodeEval adopts an execution-based evaluation and offers a multilingual code execution engine, ExecEval that supports unit test based execution in all the $11$ languages. To address the challenge of balancing the distributions of text-code samples over multiple attributes in validation/test sets, we propose a novel data splitting and a data selection schema based on the geometric mean and graph-theoretic principle. Our experiments with OpenAI's LLMs (zero-shot) and open-LLMs (zero-shot and fine-tuned) on the tasks and languages demonstrate **xCodeEval** to be quite challenging as per the current advancements in language models.

==> sections/51_acknowledgement.tex <==
We want to thank Asst. Prof. Dr. Md Moniruzzaman from the Islamic University of Technology for his contribution to the early phase of the project. 

==> tables/apr_alg.tex <==
\begin{algorithm}[tb]
    \caption{APR Dataset Creation Algorithm}
    \label{alg:apr}
\begin{algorithmic}
    \STATE {\bfseries Input:} A dataset $\mathcal{D}$, a fraction value $\gamma$ where $0\le \gamma\le 1$, a integer $T$ and threshold $p = 1e^{-5}$ 
    \STATE {\bfseries Output:} $\mathcal{D}_{valid}$, $\mathcal{D}_{test}$
    \STATE {\bfseries Initialize:} $count=0, bestScore=\gamma + 1$
    \WHILE{$count < T$ and $bestScore > p$}
        \STATE $seed=getSeed()$ \hfill\COMMENT {Get a random seed for the run}
        \STATE shuffle $\mathcal{D}$
        \STATE $\mathcal{D}_{\text{valid}}$ = $\mathcal{D}[0:|\mathcal{D}| \times \gamma ]$
        \STATE Let $T_{\text{valid}}$ = set of tags in $\mathcal{D}_{\text{valid}}$ 
        \STATE $\mathcal{D}_{\text{test}}$ = $\mathcal{D}[|\mathcal{D}| \times \gamma : |\mathcal{D}| ]$
        \STATE Let $T_{\text{test}}$ = set of tags in $\mathcal{D}_{\text{test}}$
        \IF{$T_{\text{valid}} \neq T_{test}$}{
            \STATE continue
        }
        \ENDIF
        \FORALL{t in $T_{\text{valid}}$}{
   		    \STATE x = \#samples in $\mathcal{D}_{\text{valid}}$ have tag t
   		    \STATE y = \#samples in $\mathcal{D}_{\text{test}}$ have tag t
   		    \STATE  $\alpha_t \leftarrow x/y$
   		}
        \ENDFOR
        \STATE $\alpha$ = $geoMean(\alpha_{t \in {T_{\text{valid}}}})$
        \IF{$|\gamma-bestScore| > |\gamma-\alpha|$}{
   		   \STATE $bestScore$ = $\alpha$ 
   		   \STATE save current split $\{\mathcal{D}_{\text{valid}}$, $\mathcal{D}_{\text{test}}\}$
      	   \STATE $count = count + 1$
   		}
        \ENDIF
    \ENDWHILE

\end{algorithmic}
\end{algorithm}

==> tables/datasets_small.tex <==
\begin{table*}
\centering
\caption{\small Comparison between \tool  and other benchmarks. For simplicity, we combine NL-code generation and code completion as Program Synthesis.
% and can also be used code summarization. 
Compared to others, \tool offers the largest suite of training and test data and a more comprehensive set of test cases. Evaluation levels \texttt{Global}, \texttt{Modular}, and \texttt{Local} refer to document, function, and statements level evaluation, respectively. A more detailed version of this table can be found in Appendix \ref{appendix:related-work} of supp. material.
}
%\vspace{3mm}
\label{tab:dataset-comparision}
% \resizebox{16cm}{!} 
\resizebox{0.95\linewidth}{!}
{
\begin{tabular}{l|rrclllll}
\toprule
Dataset & |Train|  & |Test| & |La| & Task Type & Evaluation & Level & Genre\\ \midrule
% Django \citep{django} & 16,000 & 1,805 & 1 & Program Synthesis & Lexical & Local & N/A\\ 
% WikiSQL \citep{zhongSeq2SQL2017} & 56,355 & 15,878 & 1 & SQL Queries & Lexical & Modular & SQL\\
% \citet{miceli-barone-sennrich-2017-parallel} & 109,108 & 2,000 & 1 & Synthesis, Summarization & Lexical & Local & Github \\
% CoNaLa  \citep{CoNaLa} & 2,379  &  500  & 2 & Program Synthesis & Lexical & Local  & Stackoverflow: QA\\
% CONCODE \citep{concode} & 100,000 & 2,000 & 1 & Program Synthesis & Lexical & Modular & Github \\
% Android \citep{parvez2018building} & 26,600 & 3,546 & 1 & Program Synthesis & Lexical & Local & Map oriented, GitHub \\
% CodeSearchNet \citep{codesearchnet} &  6,452,446 & 99 & 6 & Plain Text, Retrieval & NDCG & Modular & Github\\
% JuICe  \citep{agashe2019juice} & 1,518,049  & 1,981 & 1 & Notebook Cell Gen. & Lexical & Local & Prog. assignment\\
% TransCoder \citep{roziere2020unsupervised} & 721MB & 1,410 & 3 & Program Translation & Lexical & Modular & Github\\
HumanEval  \citep{codex} & -  & 164 & 1 & Program Synthesis & Execution & Modular & Interview Question\\
HumanEval-X\citep{humaneval-x} & -  & 820 & 9 &  Synthesis \& Translation & Execution & Modular & Interview Question\\
MBPP  \citep{mbpp} & -  & 974 & 1 & Program Synthesis & Execution & Modular & Interview Question \\
CodeXGLUE   \citep{codexglue} & 2,840,000 & 759,000 & 9 & 10 Tasks & Lexical & Local & N/A\\
% AVATAR \citep{ahmad2021avatar} & 5,937 & 1,693 & 2 & Program Translation & Lexical & Global & Problem Solving\\
% TFix \citep{tfix} & 84,846 & 10,504 & 1 & Program Repair & Lexical & Local & Github\\
% CCSD \citep{liu2021retrievalaugmented}  &  84,316 & 6,533 & 1 & Program Summarization & Lexical & Modular & Linux Kernel  \\
% TL-CodeSum~\citep{TLCODESUM} & 55,766  & 6,971 & 1& Program Summarization &  Lexical & Modular & Github \\
% Python-Sum~\citep{miceli-barone-sennrich-2017-parallel} & 55,538 & 18,502 & 1 & Program Summarization & Lexical & Modular & Github\\
% CodeNet \citep{puri2021codenet} & 8,906,769 & 2,783,365 & 55 &  Classification, similarity & Lexical & Global & Problem Solving \\
% TransCoder-ST \citep{roziere2021leveraging} &  333,542 & 103,488 & 3 & Program Translation & Execution & Modular & Github\\
% DSP  \citep{chandel2022training} & -  & 1,119  & 1 & Notebook Cell Gen. & Execution & Local & Math and Data Science \\
MTPB  \citep{codegen} & -  & 115  & 1 & Multi-turn Code Gen. & Execution & Local & Problem Solving \\
% Exe-DS \citep{huang2022execution} & 119,266  & 534  & 1 & Notebook Cell Gen. & Execution & Local & Data Science \\
DS-1000 \citep{lai2022ds} & -  &  1,000  & 1 & Notebook Cell Gen. & Execution & Local & Data Science \\
% MoCoNaLa \citep{wang2022mconala} & -  &  896  & 1 & Program Synthesis & Lexical & Local & StackOverflow \\
% ARCADE \citep{yin2022natural} & -  &  1082  & 1 & Notebook Cell Gen. & Lexical & Local & Data Science \\
ODEX \citep{wang2022execution} & - & 945 & 1 & 
% NL to code Generation 
Program Synthesis
& Execution & Local & StackOverflow\\
MBXP \citep{mbxp_athiwaratkun2022} &  -  & 13,877  & 10 & Program Synthesis & Execution & Modular & Interview Question\\
XLCoST\citep{zhu2022xlcost} & 496,333 & 45,394 & 7 & 10 Task & Lexical & Local, Global & GitHub\\
\midrule
DeepFix~\citep{gupta2017deepfix} & 37,000 & 7000 & 1 & Program Repair & Ececution & Global & Compile Error, Students\\
Defects4J \citep{defects4js} & - & 835 & 1 & Program Repair & Execution & Local, Global & N/A \\
APPS \citep{apps} & 5,000  & 5,000  & 1 & Program Synthesis & Execution & Global & Interview Question\\
CodeContests \citep{code_contest} & 4,432,447  & 32,181  & 3 & Program Synthesis & Execution & Global & Problem Solving\\
CoderEval \citep{yu2023codereval} & - & 460 & 2 & Program Synthesis & Execution & Modular,  Global & GitHub\\
\midrule
{\bf \toolnospace} (ours) & 19,915,150 & 159,464 & 17 & 7 Tasks, see Table \ref{tab:data-stat} & Execution & Global & Problem Solving \\
\bottomrule
\end{tabular}
}
% \vspace{-2em}
\end{table*}


==> tables/lang-version-support-execeval.tex <==
\begin{table*}[!htb]
\centering
\caption{Supported languages and their versions in \texttt{ExecEval}.}
\label{tab:supported-langs}
% \small
% \scriptsize 
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|l}
    \hline
    Language & compiler & Supported Versions \\
    \hline 
    Ruby & ruby 3.0.2p107 & Ruby 3 \\
    Javascript & node.js v16.17.1 & Node.js v16.17.1 \\
    Go & go1.19.2 & Go 1.19 \\
    C++ & gcc 12.1.0 & GNU C++17, GNU C++20, GNU C++11, GNU C++14, GNU C++17, GNU C++0x\\
    & clang 14.0.0 & Clang++17, Clang++20 \\
    C & gcc 12.1.0 & GNU C11, GNU C \\
    Java & java 19.0.2 & Java 6, Java 7, Java 17, Java 11, Java 8 \\
    Python & PyPy 7.3.9 with GCC 10.2.1 & PyPy 3.9.12, PyPy 2.7.18,  \\
    & Python 2.7.18 & Python 2.7.18 \\
    & Python 3.11.0rc1 & Python 3.11 \\
     C\# & Mono JIT compiler version 6.12.0.182 & Mono C\# 6.12 \\
    PHP & PHP 8.1.2 & PHP 8.1 \\
    Rust & rustc 1.67.1 & Rust 2021, Rust 2018, Rust 2015 \\
    Kotlin & Kotlin 1.7.20 & Kotlin 1.7.20 \\
    \hline
\end{tabular}
}

\end{table*}

==> tables/tags_results.tex <==
% \begin{table*}[]
% \scalebox{0.95}{
% \begin{tabular}{l|rrrrrrrrrrr|l}
% \hline
% Model & C & C\# & C++ & Go & Java & Javascript & Kotlin & PHP & Python & Ruby & Rust & Ave. \\ \hline
% \multicolumn{12}{c}{\textbf{Code2Tag}}  \\
% % RoBERTa & - & - & - & - & - & - & - & - & - & - & - & - \\
% CodeBERT & x & x & x & - & - & - & x & - & - & - & x & - \\
% % PLBart & - & - & - & - & - & - & - & - & - & - & - & - \\
% CodeT5 & - & - & - & - & - & - & - & - & - & - & - & - \\
% \hline
% \multicolumn{12}{c}{\textbf{DesCode2Tag}}  \\
% % RoBERTa & - & - & - & - & - & - & - & - & - & - & - & - \\
% CodeBERT & x & x & x & - & - & - & x & - & - & - & x & - \\
% % PLBart & - & - & - & - & - & - & - & - & - & - & - & - \\
% CodeT5 & - & - & - & - & - & - & - & - & - & - & - & - \\
% \hline
% \end{tabular}
% }
% \caption{Tag classification results (MCC)}
% \end{table*}

==> tables/tags_tokens.tex <==
% \begin{table}[h]
% \centering
% \small
% \scalebox{1}{\begin{tabular}{l|c|c|c}
% \hline
% Type  & Train & Valid & Test   \\
% \hline
% Avg. Tags & 2.67 & 2.21 & 2.19 \\
% Avg. Characters (Code) & 1278.65 & 953.29 & 964.14 \\
% Avg. Tokens (Des) & 277.46 & 174.03 & 174.39 \\
% % Unique chars (Code) & - & - & -    \\
% % Unique tokens (Des) & - & - & - \\
% \hline
% \end{tabular}
% }
% \vspace{-2mm}
% \caption{
%     \small Linguistic statistics of the tag classification benchmark.
% }
% \vspace{-2mm}
% \label{tab:tag-classification-token-stats}
% \end{table}
